DERA: Enhancing Large Language Model Completions with Dialog-Enabled Resolving Agents

Large language models (LLMs) have emerged as valuable tools for many natural language understanding tasks. In safety-critical applications such as healthcare, the utility of these models is governed by their ability to generate outputs that are factually accurate and complete. In this work, we present dialog-enabled resolving agents (DERA). DERA is a paradigm made possible by the increased conversational abilities of LLMs, namely GPT-4. It provides a simple, interpretable forum for models to communicate feedback and iteratively improve output. We frame our dialog as a discussion between two agent types - a Researcher, who processes information and identifies crucial problem components, and a Decider, who has the autonomy to integrate the Researcher's information and makes judgments on the final output. We test DERA against three clinically-focused tasks. For medical conversation summarization and care plan generation, DERA shows significant improvement over the base GPT-4 performance in both human expert preference evaluations and quantitative metrics. In a new finding, we also show that GPT-4's performance (70%) on an open-ended version of the MedQA question-answering (QA) dataset (Jin et al. 2021, USMLE) is well above the passing level (60%), with DERA showing similar performance. We release the open-ended MEDQA dataset at https://github.com/curai/curai-research/tree/main/DERA.

==> sections/related_work.tex <==
\section{Related work}

Developments in deep learning-based large language models have been a recent focus in the field of natural language processing \cite{peters-etal-2018-deep, devlin-etal-2019-bert}.  These models are designed to build representations of text thmeaningse words with similar meaning in a similar vector space regardless of lexical form. This reduces the need for feature engineering and enables fine-tuning to text in specific domains \cite{alsentzer-etal-2019-publicly, pubmedbert}.  Building off of this approach, other large language models \cite{brown2020gpt3, lewis-etal-2020-bart} have fueled advances in generating text.  This generation capability can not only be applied to classical generation tasks, such as summarization \cite{goyal2022news,bhskar-etal-2022-opinion,sclar2022referee,narayan-etal-2021-planning}, but also tasks that traditionally required task-specific models \cite{Agrawal2022LargeLM,dou-etal-2022-gpt,gao-etal-2022-precise}.

Previously, models built on encoder-based language models (\eg BERT) required task-specifcity performance to achieve high-performance.  The ability of generative language models to create output based on natural language instructions (or prompts) removes the need for task-specific training \cite{min-etal-2020-demonstrations} and allows for non-experts to build upon this technology.  Additional research has shown that generation performance can be improved when examples of the task are included in the prompt \cite{brown2020gpt3}.  Further advanced prompting approaches include \textit{chaining} \cite{wu2022AIChains}, where subtasks are discretely processed.  This allows for interpretability at each step and allows the model to focus on specific aspects of the task.  Similarly, chain-of-thought strategies \cite{wei2022chain} prompt the model to think through a problem in a way an expert might approach it, which leads to improvements in some tasks. Some work studies training generative models to perform specific tasks (\eg soft prompt learning, \cite{qin-eisner-2021-learning}), this requires access to a set of training examples and the ability to fine-tune a model, which is currently not possible for many (\eg \LLM). 


\paragraph{Summarization}
While the task of clinical text summarization has been studied before the advent of large language models \cite{pivovarov-elhadad-2015-automated}, neural methods have consistently shown better performance \cite{liang-etal-2019-novel-system, gao-etal-2022-summarizing, macavaney2019ontology}. Much work focuses on summarizing clinician-generated data, but summarization of clinical dialog adds the challenge of understanding patient-generated text \cite{enarvi-etal-2020-generating, joshi-etal-2020-dr, zhang2021leveraging}.

\paragraph{Question Answering}
Natural language question answering has similarly been well studied in the field \cite{hovy2000question, brill-etal-2002-analysis}, with early systems focused on building pipelines to discretize the task.  Similarly to summarization, neural methods applied to the task have shown broad improvements in question-answer capability \cite{andreas-etal-2016-learning}.  This is especially true for Medical Question Answering given the complexity of the questions and the domain.  Commonly, question-answering datasets \cite{jin2021disease, palMedMCQA} consist of multiple-choice questions, where a question is paired with four or five options, and the system must select which option is the correct answer.  Other datasets \cite{Abacha2017OverviewOT} consist of open-ended questions, but are taken from health websites that do not probe as deep of knowledge as medical licensing exams. 

The creators of the MedQA dataset evaluated that dataset against many existing question-answering approaches and found that a RoBERTa-based model \cite{liu2019roberta} performed best. Recent approaches for Medical Question answering have leveraged generative LLMs to perform the task.   Other authors\cite{lievin2022can}, focus on refining chain-of-thought strategies for several medical datasets using language models such as BERT.  In \cite{singhal2022large}, the authors fine-tune an existing LLM, Plam \cite{chowdhery2022palm}, to perform well on medical tasks.  They also include some small experiments on open-ended question answering but do not perform large-scale evaluations.  In both cases, the author achieve passing results on MedQA and MedMCQA (defined as above 50\%). In all cases, the authors primarily focus on the multiple-choice question format.
Other work \cite{choi-etal-2018-quac} has studied a teacher-student format for similar tasks, but do so with crowdworkers.

==> sections/summ_experiments.tex <==
\section{Experiments}

\subsection{Care Plan Generation}
\paragraph{API Parameters and Prompts} We run DERA on the care plan generation task using GPT-4 with the settings mentioned in Table \ref{tab:summ_experimental_details}. The initial prompt for generating the care plan is found in Prompt \ref{prompt:careplan}, \Researcher prompt in Prompt \ref{}, \Decider prompt in Prompt \ref{}, and the final prompt that takes the scratchpad of suggestions from the \Researcher and outputs the final care plan is in Prompt \ref{}.

\paragraph{Dataset} Care plans are generated on 50 \TODO{update to 100} real-world tele-health encounters randomly selected within the past year of this writing. Each encounter contains the patient's age, sex, reason for visit, and chat conversation with a licensed medical provider. Each medical encounter evaluated covers a variety of patient presentations, including urinary tract infections, toothaches, headaches, abdominal pain, and others. \TODO{Include other summary statistics?}.

\paragraph{Qualitative Evaluation} To evaluate the effectiveness of DERA to generate care plans, we conducted a qualitative evaluation by asking \TODO{4} licensed physicians several questions before and after interventions made by DERA. In our study, the care plan was defined as "meant to be provider-facing, meaning that not all suggested interventions will necessarily be recommended to the patient or followed by the patient." 

The questions asked were: 1) How many of the necessary care management steps are recommended in the care plan? (Options: All, Most, Some, None) 2) If this care plan were acted upon by the patient, does this care plan contain information that could potentially be harmful to the patient given their presentation? (Yes, No).

The physicians were also asked if they agreed with the corrections added to the scratchpad, on a scale of All, Most, Some, None. Note that the physicians who evaluated the quality of these care plans were not those who provided care to the patients in the original encounter.

\subsection{Summarization}
\paragraph{API Parameters and Prompts}
\label{sec:summ_api_params}
We run DERA on the summarization task using GPT-4 with the settings mentioned in Table \ref{tab:summ_experimental_details}. For the basic \Researcher - \Decider experiments on summarization, we use prompts very similar to those used in the care plan (\Researcher: Prompt \ref{}, \Decider: Prompt \ref{}, Final Prompt: Prompt \ref{}). For experiments in which we artificially induce a corruption into the initial summary (see more below in Quantitative Evaluation), we use Prompt \ref{}. Finally, for the experiments that separate \Researcher - \Decider access to the medical dialog and medical history, we used the following prompts: \Researcher: Prompt \ref{}, \Decider: Prompt \ref{}. The final prompt used in this setup is the same as before.

\paragraph{Dataset} For our qualitiative evaluation presented below, summaries are generated on the same 50\footnote{We were only able to qualitatively evaluate 50 encounters due to limited labeling constraints.} \TODO{update to 100} real-world tele-health encounters used in the care plan experiment. As stated earlier, each encounter contains the patient's age, sex, reason for visit, and chat conversation with a licensed medical provider.

We also present quantitative results on much larger dataset of 250 \TODO{Update to 500 if possible} real-world tele-health encounters. This dataset is a superset of the encounters used previously, and share the same characteristics (identical distribution of patient presentations, length, etc.). \TODO{Include other summary statistics?}.

\paragraph{Qualitative Evaluation}
\label{sec:summ_qual_eval}
To evaluate the effectiveness of DERA to generate summaries, we conducted a qualitative evaluation similar to that used in the care plan evaluation. We asked \TODO{4} licensed physicians several questions before and after interventions made by DERA. Once again, we defined our summaries to be provider-facing (i.e. summaries used for later reference by either the same or another physician).

The questions asked were: 1) What percentage of the overal clinical information in the dialog is captured by the summary? (Options: All, Most, Some, None) 2) If this summary were acted upon by another clinical provider, does this summary contain information that could potentially be harmful to the patient given their presentation? (Yes, No).

The physicians were also asked if they agreed with the corrections added to the scratchpad, on a scale of All, Most, Some, None.

\paragraph{Quantitative Evaluation}
\label{sec:summ_quan_eval}
We also quantitatively evaluate DERA's ability to write medical summaries by measuring the degree to which DERA can identify and fix "corruptions" introduced into a medical summary. These corruptions are synthetically produced by starting with the initially generated summary, and passing one of three levels of corruption, low (3/10), medium (5/10), and high (7/10) to our corruption prompt (Prompt \ref{}). We use this corruption variable (set to either 3, 5, or 7) to introduce the desired level of corruption, which can rearrange symptoms from positives to negatives and introduce hallucinated symptoms, conditions, or other details among others. While we do not expect modules that initially produce medical summaries to be this poor, we see value in stress testing the quality of these summaries and measuring if quality can be restored. Ideally, DERA can successfully correct all corruptions introduced into the summary.

We measure the degree to which corruptions are present by using a GPT-based metric that measure medical concept coverage in the medical summary, GPT-F1 \TODO{Add citation to unreleased summarization paper}. \TODO{Add brief explanation of metric here or in appendix}.
